Can Women Break the Glass Ceiling?: An Analysis of #MeToo Hashtagged Posts on Twitter

In October 2017, there happened the uprising of an unprecedented online movement on social media by women across the world who started publicly sharing their untold stories of being sexually harassed along with the hashtag #MeToo (or some variants of it). Those stories did not only strike the silence that had long hid the perpetrators, but also allowed women to discharge some of their bottled-up grievances, and revealed many important information surrounding sexual harassment. In this paper, we present our analysis of about one million such tweets collected between October 15 and October 31, 2017 that reveals some interesting patterns and attributes of the people, place, emotions, actions, and reactions related to the tweeted stories. Based on our analysis, we also advance the discussion on the potential role of online social media in breaking the silence of women by factoring in the strengths and limitations of these platforms.

==> sec-notes.tex <==
\section{Notes}
\label{sec-notes}

The following questions appeared in our discussion.

\begin{enumerate}
    \item Compare confession of during metoo and now.
    \item Hypothesis: Attackers are most likely from close circle. How does the circle look in U.S. and in Asia?
    \item What is the gender and age \footnote{https://www.faceplusplus.com/} distribution of the tweeters/re-tweeters? \cite{bamman2014gender}
    \item What is the distribution of topics against location, gender, and age? \cite{yan2013biterm}
    \item How the \#metoo \footnote{https://en.wikipedia.org/wiki/Me\_Too\_(hashtag)} movement started and diminished?
    \item Who are the proponents of the movements? What are their demographics?
    \item What are the emotions present in the tweets and re-tweets? What is the emotion distribution against gender, age, and location? \cite{tausczik2010psychological,mohammad2013crowdsourcing,mohammad2010emotions}
    \item What kind of emotions lasts longer than the others in terms of re-twitting?
    \item What kind of harassment occurred more in what locations?
    \item What sort of discussion the metoo containing tweet creates? Further confession, sympathy, hostility?
    \item What makes a user confess or use the tag? How many from her network used the tag?
    \item At what age did the harassment happened?
    \item Who are the responsible characters? Colleague, Relative, Friends?
\end{enumerate}

Some things for future.

\begin{enumerate}
\item Can we propose a ``mixed method'' strategy to understand such web incident. By ``mixed method'', I mean ``quantitative analysis of web data'' + ``qualitative data by survey/interviewing''. I think this method will give us a broad understanding of the web phenomena like hash-tag movements and online fights. I know people already mix some qualitative factors while analyzing quantitative data, but they are often not systematic and rigorous that a qualitative researcher would do. I was wondering if we can propose something methodologically novel.

\end{enumerate}


